Session Fidelity for ElixirST: A Session-Based Type System for Elixir Modules

This paper builds on prior work investigating the adaptation of session types to provide behavioural information about Elixir modules. A type system called ElixirST has been constructed to statically determine whether functions in an Elixir module observe their endpoint specifications, expressed as session types; a corresponding tool automating this typechecking has also been constructed. In this paper we formally validate this type system. An LTS-based operational semantics for the language fragment supported by the type system is developed, modelling its runtime behaviour when invoked by the module client. This operational semantics is then used to prove session fidelity for ElixirST.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{C. Aubert, C. Di Giusto, L. Safina \& A. Scalas (Eds.):\\
15th Interaction and Concurrency Experience (ICE 2022)\\
EPTCS 365, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.365.2}{10.4204/EPTCS.365.2}}
\pdfoutput=1

